An Overview on IEEE 802.11bf: WLAN Sensing

With recent advancements, the wireless local area network (WLAN) or wireless fidelity (Wi-Fi) technology has been successfully utilized to realize sensing functionalities such as detection, localization, and recognition. However, the WLANs standards are developed mainly for the purpose of communication, and thus may not be able to meet the stringent requirements for emerging sensing applications. To resolve this issue, a new Task Group (TG), namely IEEE 802.11bf, has been established by the IEEE 802.11 working group, with the objective of creating a new amendment to the WLAN standard to meet advanced sensing requirements while minimizing the effect on communications. This paper provides a comprehensive overview on the up-to-date efforts in the IEEE 802.11bf TG. First, we introduce the definition of the 802.11bf amendment and its formation and standardization timeline. Next, we discuss the WLAN sensing use cases with the corresponding key performance indicator (KPI) requirements. After reviewing previous WLAN sensing research based on communication-oriented WLAN standards, we identify their limitations and underscore the practical need for the new sensing-oriented amendment in 802.11bf. Furthermore, we discuss the WLAN sensing framework and procedure used for measurement acquisition, by considering both sensing at sub-7GHz and directional multi-gigabit (DMG) sensing at 60 GHz, respectively, and address their shared features, similarities, and differences. In addition, we present various candidate technical features for IEEE 802.11bf, including waveform/sequence design, feedback types, as well as quantization and compression techniques. We also describe the methodologies and the channel modeling used by the IEEE 802.11bf TG for evaluation. Finally, we discuss the challenges and future research directions to motivate more research endeavors towards this field in details.

==> data/References.tex <==
\begin{thebibliography}{99}
	\bibitem{WiFi_Alliance} Telecom Advisory Services, LLC, ``The economic value of Wi-Fi: A global view (2021 and 2025),'' Sep. 2021.
	
	
	\bibitem{RSSI1} S. Yiu, M. Dashti, H. Claussen, and F. Perez-Cruz, ``Wireless RSSI fingerprinting localization,'' Signal Processing, vol. 131, pp. 235--244, Feb. 2017.
	
	\bibitem{RSSItoCSI} Z. Yang, Z. Zhou, and Y. Liu, ``From RSSI to CSI: Indoor localization via channel response,'' \textit{ACM Comput. Surv.}, vol. 46, no. 25, pp. 1--32, Dec. 2013.
	
	\bibitem{survey_ILS} F. Zafari, A. Gkelias, and K. K. Leung, ``A survey of indoor localization systems and technologies,'' {\it IEEE Commun. Surv. Tutor.}, vol. 21, no. 3, pp. 2568--2599, Apr. 2019.
	\bibitem{RSSI_fingerprint} V. Honkavirta, T. Perala, S. Ali-Loytty, and R. Piche, ``A comparative survey of WLAN location fingerprinting methods,'' in {\it Proc. 6th WPNC}, pp. 243–251, Mar. 2009.
	\bibitem{RSSI_PL_model} P. Kumar, L. Reddy, and S. Varma, ``Distance measurement and error estimation scheme for RSSI based localization in wireless sensor networks,'' in {\it Proc. 5th IEEE Conf. Wireless Commun. Sensor Netw. (WCSN)}, pp. 1--4, Dec. 2009.
	
	\bibitem{CSI_survey} Y. Ma, G. Zhou, and S. Wang, ``Wifi sensing with channel state information: A survey,'' \textit{ACM Comput. Surv.}, vol. 52, no. 3, Jun. 2019.
	
	\bibitem{SENS_tutorial} Z. Yang, Y. Zhang, G. Chi, and G. Zhang, ``Hands-on wireless sensing with Wi-Fi: A tutorial,'' Jun. 2022. [Online] Available: https://arxiv.org/abs/2206.09532
	
	\bibitem{ESPRIT} R. Roy and T. Kailath, ``Esprit-estimation of signal parameters via rotational invariance techniques,'' \textit{Acoustics, Speech and Signal Processing, IEEE Transactions on}, vol. 37, no. 7, pp. 984--995, 1989.
	\bibitem{MUSIC} R. Schmidt, ``Multiple emitter location and signal parameter estimation,'' \textit{IEEE Trans. Antennas Propag.}, vol. 34, no. 3, pp. 276--280, Mar. 1986.
	\bibitem{SAGE} J. A. Fessler and A. O. Hero, ``Space-alternating generalized expectation-maximization algorithm,'' \textit{IEEE Trans. Signal Process.}, vol. 42, no. 10, pp. 2664--2677, Oct. 1994.
	
	\bibitem{cognitive} Cognitive, [Online] Available: https://www.cognitivesystems.com/
	\bibitem{originwireless} Originwireless, [Online] Available: https://www.originwirelessai.com/
	
	\bibitem{phase_error} Y. Xie, Z. Li, and M. Li, ``Precise power delay profiling with commodity Wi-Fi,'' {\it IEEE Trans Mob Comput}, vol. 18, no. 6, pp. 1342--1355, Jun. 2019.
	
	\bibitem{11az_PAR} J. Segev, P. Thornycroft, D. Stanley, Q. Wang, B. Hart, S. Pandey, N. Kakani, J. Roshdahl, G. Venkatesan, L. Chu, E. Au, G. Bajko, C. Wang, M. Rison, F. Tang, C. Aldana, P. Dua, and M. Wang, ``NGP PAR Draft,'' IEEE 802.11-15/0030r9, Jul. 2015. [Online] Available: https://mentor.ieee.org/802.11/dcn/15/11-15-0030-09-0ngp-ngp-par-draft.docx
	
	\bibitem{ISAC} F. Liu, Y. Cui, C. Masouros, J. Xu, T. X. Han, Y. C.Eldar, and S. Buzzi. ``Integrated sensing and communications: Towards dual-functional wireless networks for 6G and beyond.'' [Online] Available: https://arxiv.org/abs/2108.07165
	
	\bibitem{ISAC2} H. Hua, X. Song, Y. Fang, T. X. Han, and J Xu, ``MIMO integrated sensing and communication with extended target: CRB-rate tradeoff,'' [Online] Available: https://arxiv.org/abs/2205.14050
	\bibitem{ISAC4} H. Hua, J. Xu, and T. X. Han, ``Optimal transmit beamforming for integrated sensing and communication,'' [Online] Available: https://arxiv.org/abs/2104.11871
	
	\bibitem{VLP1} M. F. Keskin, A. D. Sezer, and S. Gezici, ``Localization via visible light systems,'' in {\it Proc. IEEE}, vol. 106, no. 6, pp. 1063--1088, Jun. 2018.
	\bibitem{VLP2} J. Zhang, C. Zhang, X. Zhang, and S. Banerjee, ``Towards a visible light network architecture for continuous communication and localization,'' {\it  Proc. of ACM VLCS}, pp. 49--54, Oct. 2016.
	\bibitem{VLP3} S. Zhu and X. Zhang, ``Enabling high-precision visible light localization in today's buildings,'' in {\it Proc. of ACM MobiSys}, pp. 96--108, Jun. 2017.
	
	\bibitem{UPS1} X. Luo, H. Wang, S. Yan, J. Liu, Y. Zhong, and R. Lan, ``Ultrasonic localization method based on receiver array optimization schemes,'' {\it INT J DISTRIB SENS N}, vol. 14, no. 11, Nov. 2018.
	\bibitem{UPS2} Q. Lin, Z. An, and L. Yang, ``Rebooting ultrasonic positioning systems for ultrasound-incapable smart devices,'' in {\it Proc. of ACM MobiSys}, pp. 1--16, Aug. 2019.
	
	\bibitem{RFID1} A. Motroni, A. Buffi, and P. Nepa, ``A survey on indoor vehicle localization through RFID technology,'' {\it IEEE Access}, vol. 9, pp. 17921--17942, Jan. 2021.
	\bibitem{RFID2} J. Han, C. Qian, X. Wang, D. Ma, J. Zhao, W. Xi, Z. Jiang, and Z. Wang, ``Twins: Device-free object tracking using passive tags,'' {\it IEEE ACM Trans Netw}, vol. 24, no. 3, pp. 1605--1617, Jun. 2016.
	
	\bibitem{UWB} A. Alarifi, A. Al-Salman, M. Alsaleh, A. Alnafessah, S. Al-Hadhrami, M.
	A. Al-Ammar, and H. S. Al-Khalifa, ``Ultra wideband indoor positioning
	technologies: Analysis and recent advances,'' {\it Sensors}, vol. 16, no. 5, p.
	707, May 2016.
	
	\bibitem{Intel5300} Linux 802.11n CSI Tool, [Online] Available: https://dhalperi.github.io/linux-80211n-csitool/
	
	\bibitem{AR9589} Atheros-CSI-Tool, [Online] Available: https://wands.sg/research/wifi/AtherosCSI/Hardware.html
	
	
%	\bibitem{11bfwork} R. Francesco. ``IEEE 802.11 bf: Toward ubiquitous Wi-Fi sensing,'' Mar. 2021. [Online] Available: https://arxiv.org/abs/2103.14918
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	
	
	\bibitem{WNG_SEN1} T. X. Han, R. Du, C. Liu, M. Zhang, and D. X. Yang, ``Wi-Fi sensing,'' IEEE 802.11-19/1164r0, Jul. 2019. [Online] Available: https://mentor.ieee.org/802.11/dcn/19/11-19-1164-00-0wng-wi-fi-sensing.pptx
	\bibitem{WNG_SEN2} C. da Silva, C. Cordeiro, B. Sadeghi, C. Chen, and A. Lomayev, ``Wi-Fi sensing: Usages, requirements, technical feasibility and standards gaps,'' IEEE 802.11-19/1293r0, Jul. 2019.
	\bibitem{WNG_SEN3} T. X. Han, R. Du, B. Zhou, X. Peng, Z. Rong, P. Zhang, J. Luo, C. Liu, M. Zhang, D. Shang, J. Li, D. X. Yang, X. Zuo, K. Meng, G. X. Hu, and X. Dong, ``Wi-Fi sensing - Follow up,'' IEEE 802.11-19/1500r0, Jul. 2019.
	
	
	\bibitem{SENS_SG} IEEE 802.11, Status of IEEE 802.11 WLAN Sensing (SENS) SG, [Online] Available: https://www.ieee802.org/11/Reports/senstig$\_$update.htm
	
	\bibitem{11bf_PAR} C. Silva, ``802.11 SENS SG Proposed PAR,'' IEEE 802.11-19/2103r12, Aug. 2020.
	\bibitem{11bf_use_case} A. Kasher, A. Eitan, S. Trainin, Y. Sun, and R. Du, ``WiFi sensing use cases,'' IEEE 802.11-21/1712r2, Jan. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/20/11-20-1712-02-00bf-wifi-sensing-use-cases.xlsx
	
	\bibitem{802.11_specif} IEEE, `IEEE standard for information technology--telecommunications and information exchange between systems - local and metropolitan area networks--specific requirements - part 11: Wireless LAN medium access control (MAC) and physical layer (PHY) specifications,'' in \textit{IEEE Std 802.11-2020 (Revision of IEEE Std 802.11-2016)} , vol., no., pp.1--4379, Feb. 2021.

	
	\bibitem{11bf_passive_ABFT} Narengerile, R. Du, M. Hu, Y. Xin, and A. Kasher, ``DMG passive sensing based on A-BFT,'' IEEE 802.11-22/0423r0, Mar. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/22/11-22-0423-00-00bf-dmg-passive-sensing-based-on-a-bft.pptx
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Use Cases %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bibitem{11bf_KPI} Y. Sun, D. K. P. Tan, R. Du, C. Liu, M. Zhang, and E. Au, ``Usage model terminology for WLAN sensing,'' IEEE 802.11-20/0905r2, Jun. 2020. [Online] Available: https://mentor.ieee.org/802.11/dcn/20/11-20-0905-02-SENS-usage-model-terminology-for-wlan-sensing.pptx
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Human Target Localization and Tracking
	\bibitem{ref1} F. K. Chuah, and S. S. Teoh, ``Thermal sensor based human presence detection for smart home application,'' in \textit{IEEE Int. Conf. Control Syst. Comput. Eng.}, pp. 37--41, Aug. 2020.
	\bibitem{ref2} D. Deiana, E. M. Suijker, R. J. Bolt, A. P. M. Maas, W. J. Vlothuizen, and A. S. Kossen, ``Real time indoor presence detection with a novel radar on a chip,'' in \textit{2014 International Radar Conference}, pp. 1--4, Oct. 2014.
	
	\bibitem{TRRS} K. J. R. Liu and B. Wang, ``Wireless AI: Wireless sensing, positioning, IoT, and communications.'' Cambridge, U.K.: Cambridge Univ. Press,2019.
	
	\bibitem{WiSH} T. Hang, Y. Zheng, K. Qian, C. Wu, Z. Yang, X. Zhou, Y. Liu, and G. Chen,``WiSH: WiFi-based real-time human detection,'' \textit{Tsinghua Science and Technology}, vol. 24, no. 5, pp. 615--629, Oct. 2019. 
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Activites Recognition
	\bibitem{wifi isac challenges} D. Zhang, D. Wu, K. Niu, X. Wang, F. Zhang, J. Yao, D. Jiang, and F. Qin, `` Practical issues and challenges in CSI-based integrated sensing and communication,'' [Online] Available: https://arxiv.org/abs/2204.03535
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Human Target Localization and Tracking
	\bibitem{localization} F. Zafari, A. Gkelias, and K. K. Leung, ``A survey of indoor localization systems and technologies,'' \textit{IEEE Commun. Surveys Tuts.}, vol. 21, no. 3, pp. 2568--2599, Apr. 2019.
	
	\bibitem{Chronos} D. Vasisht, S. Kumar, and D. Katabi, ``Decimeter-level localization with a single WiFi access point,'' in \textit{Proc. 13th USENIX Symp. Netw. Syst. Design Implement. (NSDI)}, 2016, pp. 165–178.
	
	
	\bibitem{IndoTrack} X. Li, D. Zhang, Q. Lv, J. Xiong, S. Li, Y. Zhang, and H. Mei, ``IndoTrack: Device-free indoor human tracking with commodity Wi-Fi,'' \textit{Proc ACM Interact Mob Wearable Ubiquitous Technol.}, vol. 1, no. 72, pp. 1--22, Sep. 2017.
	
	\bibitem{Widar2} K. Qian, C. Wu, Y. Zhang, G. Zhang, Z. Yang, and Y. Liu,  ``Widar2.0: Passive human tracking with a single Wi-Fi link,'' in \textit{Proc. 16th Annu. Int. Conf. Mobile Syst. Appl. Services}, pp. 350--361, Jun. 2018.
	
	\bibitem{SAGE_short} R. Yang, X. Yang, J. Wang, M. Zhou, Z. Tian, and L. Li, ``Decimeter level indoor localization using WiFi channel state information,'' \textit{IEEE Sens. J.}, vol. 22, no. 6, pp. 4940--4950, Mar. 2022.
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Healthcare Analysis
	\bibitem{Wi-Sleep} X. Liu, J. Cao, S. Tang, and J. Wen, ``Wi-Sleep: Contactless sleep monitoring via WiFi signals,'' in \textit{Proc. IEEE Real-Time Systems Symposium}, pp. 346--355, Dec. 2014.
	\bibitem{TVS} J. Liu, Y. Wang, Y. Chen, J. Yang, X. Chen, and J. Cheng, `` Tracking vital signs during sleep leveraging off-the-shelf wifi,'' in \textit{Proc. 16th ACM Int. Symp. Mobile Ad Hoc Netw. Comput.}, pp. 267--276, Jun. 2015.
	\bibitem{PhaseBeat} X. Wang, C. Yang, and S. Mao, ``PhaseBeat: Exploiting CSI phase data for vital sign monitoring with commodity WiFi devices,'' in \textit{Proc. IEEE 37th Int. Conf. Distrib. Comput. Syst.}, pp. 1230--1239, Jun. 2017.
	\bibitem{MultiSense} Y. Zeng, D. Wu, J. Xiong, J. Liu, Z. Liu, and D. Zhang, ``MultiSense: Enabling multi-person respiration sensing with commodity WiFi,'' in \textit{Proc. ACM Interactive, Mobile, Wearable Ubiquitous Technol.}, no. 102, pp. 1--29, Sep. 2020.
	\bibitem{Wi-Sneeze} D. K. P. Tan \textit{et al}., ``Wi-Sneeze- Sneeze sensing using Wi-Fi signals,'' in \textit{2020 IEEE Globecom Workshops (GC Wkshps}, pp. 1--6, Dec. 2020.
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% 3D Vision
	\bibitem{openpose} OpenPose, [Online] Available: https://github.com/CMU-Perceptual-Computing-Lab/openpose
	\bibitem{mmwave_mapping} C. B. Barneto, E. Rastorgueva-Foi, M. F. Keskin, T. Riihonen, M. Turunen, J. Talvitie, H. Wymeersch, and M. Valkama, ``Millimeter-wave mobile sensing and environment mapping: Models, algorithms and validation,'' \textit{IEEE Trans. Veh. Technol.}, vol. 71, no. 4, pp. 3900--3916, Apr. 2022.
	\bibitem{slam} E. Leitinger, F. Meyer, F. Hlawatsch, K. Witrisal, F. Tufvesson, and M. Z. Win, ``A belief propagation algorithm for multipath-based SLAM,'' \textit{IEEE Trans. Wirel. Commun.}, vol. 18, no. 12, pp. 5613--5629, Dec. 2019.
	\bibitem{rf_skeleton} M. Zhao, Y. Tian, H. Zhao, M. A. Alsheikh, T. Li, R. Hristov, Z. Kabelac, D. Katabi, and A. Torralba, ``RF-based 3D skeletons,'' in  \textit{Proceedings of the 2018 Conference of the ACM Special Interest Group on Data Communication}, Aug. 2018.
	\bibitem{person_in_wifi} F. Wang, S. Zhou, S. Panev, J. Han, and D. Huang, ``Person-in-WiFi: Fine-grained person perception using WiFi,'' in \textit{Proceedings of the IEEE/CVF International Conference on Computer Vision}, 2019.
	\bibitem{wipose} W. Jiang, H. Xue, C. Miao, S. Wang, S. Lin, C. Tian, S. Murali, H. Hu, Z. Sun, and L. Su, ``Towards 3D human pose construction using WiFi,'' in \textit{Proceedings of the 26th Annual International Conference on Mobile Computing and Networking}, Apr. 2020.
	
	
	%%%%%%%%%% Procedure
	
	\bibitem{11bf_NonTB_instan} C. Chen, D. Das, and C. Cordeiro, ``Non-TB sensing measurement,'' IEEE 802.11-21/1433r2, Aug. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-1433-02-00bf-non-tb-sensing-measurement.pptx
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Network Sensing %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	\bibitem{11bf_NetSENS_Feas} C. Silva, C. Cordeiro, B. Sadeghi, A. Lomayev, C. Chen, G. Venkatesan, and P. Hunt, ``Wi-Fi sensing: Cooperation and standard support,'' IEEE 802.11-19/1416r0, Aug. 2019. [Online] Available: https://mentor.ieee.org/802.11/dcn/19/11-19-1416-00-0wng-wi-fi-sensing-cooperation-and-standard-support.pptx
	
%	\bibitem{Data_association} Q. Shi, L. Liu, S. Zhang, and S. Cui, ``Device-free sensing in OFDM cellular network,'' {\it IEEE J. Sel. Areas Commun.}, vol. 40, no. 6, pp. 1838--1853, Jun. 2022.
%	\bibitem{Limits_DeviceBased} A. Liu, Z. Huang, M. Li, Y. Wan, W. Li, T. X. Han, C. Liu, R. Du, D. K. P. Tan, J. Lu, Y. Shen, F. Colone, and K. Chetty, ``A survey on fundamental limits of integrated sensing and communication,'' {\it IEEE Commun. Surv. Tutor.}, vol. 24, no. 2, pp. 994--1034, Feb. 2022.
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Waveform/Sequence %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bibitem{11bf_sequence} R. Du, D. T. K. Pin, M. Zhang, C. Liu, and Y. Sun, ``Discussion on WLAN sensing sequence design - follow up,'' IEEE 802.11-20/1529r0, Sep. 2020. [Online] Available: https://mentor.ieee.org/802.11/dcn/20/11-20-1529-00-SENS-discussion-on-wlan-sensing-sequence-design-follow-up.pptx
	\bibitem{Ambiguity} M. I. Skolnik, ``Introduction to radar systems.'' \textit{New York}, 1980.
	\bibitem{802.11ay} IEEE 802.11 Working Group. ``Enhanced throughput for operation in license-exempt bands above 45 GHz.'' \textit{IEEE P802. 11ay D}, 2017.
	\bibitem{LAZ/ZAZ} Z. Ye, Z. Zhou, P. Fan, Z. Liu, X. Lei, and X. Tang, ``Low ambiguity zone: Theoretical bounds and doppler-resilient sequence design in integrated sensing and communication systems,'' \textit{IEEE J. Sel. Areas Commun.}, vol. 40, no. 6, pp. 1809--1822, Jun. 2022.
	\bibitem{11bf_Sync} A. Kasher, ``PDT EDMG multi-static PPDU structure,'' IEEE 802.11-22/0464r6, Mar. 2022. [Online] Available: https://mentor.ieee.org/802.11/dcn/22/11-22-0464-06-00bf-pdt-edmg-multi-static-ppdu-structure.docx
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Feedback %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bibitem{11bf_PartialCSI} R. Chitrakar, R. Pushkarna, Y. Ding, Y. Urabe, and H. Motozuka, ``Partical CSI feedback,'' IEEE 802.11-21/1921r1, Nov 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-1921-01-00bf-partial-csi-feedback.pptx
	\bibitem{11bf_TCIR} R. Du, C. Liu, M. Zhang, Y. Sun, and D. K. P. Tan, ``Truncated power delay profile,'' IEEE 802.11-21/0660r0, May 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-0660-00-00bf-truncated-power-delay-profile.pptx
	\bibitem{11bf_DifferQuanti} Q. Li, H. Song, X. Chen, C. Chen, and R. Stacey, ``Differential quantization for CSI report,'' IEEE 802.11-21/0506r1, Mar. 2022. [Online] Available: https://mentor.ieee.org/802.11/dcn/22/11-22-0506-01-00bf-differential-quantization-for-csi-report.pptx
	
	\bibitem{11bf_SensingImage} A. Eitan, A. Kasher, and S. Trainin, ``Imaging radar data report,'' IEEE 802.11-21/1801r2, Nov. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-1801-02-00bf-imaging-radar-data-report.pptx
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Quantization %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bibitem{802.11-2012} IEEE 802.11 Working Group, ``IEEE standard for information technology-telecommunications and information exchange between systems-local and metropolitan area networks-specific requirements part 11 : Wireless LAN medium access control (MAC) and physical layer (PHY) specifications,'' IEEE Std, Feb. 2012.
	
	\bibitem{11bf_SimplScaling} J. Suh, Y. Xin, O. AboulMagd, and E. Au, ``Simplified scaling factor feedback for CSI matrices quantization,'' IEEE 802.11-21/1676r1, Oct. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-1676-01-00bf-simplified-scaling-factor-feedback-for-csi-matrices.pptx
	
	\bibitem{11bf_LowScaling} S. Shellhammer B. Tian, A. Raissinia, and S. Merlin, ``Low-complexity scaling and quantization for CSI report,'' IEEE 802.11-21/1573r1, Oct. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-1573-01-00bf-low-complexity-scaling-and-quantization-for-csi-report.pptx
	
	\bibitem{11bf_FracScaling} S. Shellhammer, A. Raissinia, and B. Tian, ``Fractional scaling factor for sensing measurement report,'' IEEE 802.11-22/0414r2, Mar. 2022. [Online] Available: https://mentor.ieee.org/802.11/dcn/22/11-22-0414-02-00bf-fractional-scaling-factor-for-sensing-measurement-report.pptx
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Security and Privacy %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bibitem{SecurityReq} M. Montemurro, ``Sensing security requirements,'' IEEE 802.11-22/0401r4, Apr. [Online] Available:  2022.https://mentor.ieee.org/802.11/dcn/22/11-22-0401-04-00bf-sensing-security-requirements.pptx
	
	\bibitem{TG4ab_UBW_Privacy} L. Sun, P. Liu, and D. X. Yang, ``Privacy issues in UWB sensing,'' IEEE 802.15-22/0177r0, Mar. 2022. [Online] Available:  https://mentor.ieee.org/802.15/dcn/22/15-22-0177-01-04ab-privacy-issues-in-uwb-sensing.pptx
	
	\bibitem{CSI_Fuzzer} X. Jiao, M. Mehari, W. Liu, M. Aslam, and I. Moerman, ``Openwifi CSI fuzzer for authorized sensing and covert channels,'' in {\it Proc., ACM Conference on Security and Privacy in Wireless and Mobile Networks (WiSec)}, NY, USA, pp. 377--379, Jun. 2021.
	\bibitem{11bf_Encrypted_TRN} R. Du, Narengerile, M. Hu, S. McCann, and M. Montemurro, ``Encrypted measurement in WLAN sensing at 60GHz,'' IEEE 802.11-22/0544r0, Mar. 2022. [Online] Available:  https://mentor.ieee.org/802.11/dcn/22/11-22-0544-00-00bf-encrypted-measurement-in-wlan-sensing-at-60ghz.pptx
	
	
	%%%%%%%%%%%%%%%%%%%%%%%%%% Simulation and Channel Model %%%%%%%%%%%%%%%%%%%%%%%%%%%%
	\bibitem{11bf_evaluation} R. Du, M. Zhang, Y, Lv, M. Hu, K. S. Au, Y. Xin, J. Suh, O. AboulMagd, H. Dai, S. Shi, W. Wang, Y. Shen, J. Xu, and F. Liu, ``11bf evaluation methodology and simulation scenarios,'' IEEE 802.11-21/0876r3, Sep. 2021. [Online] Available:  https://mentor.ieee.org/802.11/dcn/21/11-21-0876-03-00bf-11bf-evaluation-methodology-and-simulation-scenarios.doc
	
	\bibitem{SENS_evaluation} R. Du, M. Zhang, C. Liu, Y. Sun, D. K. P. Tan, and E. Au, ``Discussion on WLAN sensing evaluation methodology,'' IEEE 802.11-20/0907r1, Jul. 2020. [Online] Available:  https://mentor.ieee.org/802.11/dcn/20/11-20-0907-01-SENS-discussion-on-wlan-sensing-evaluation-methodology.pptx
	
	\bibitem{11ax_evaluation} R. Porat {\it et al}, ``Evaluation methodology,'' IEEE 802.11-14/0571r12, Jan. 2016. [Online] Available:  https://mentor.ieee.org/802.11/dcn/14/11-14-0571-12-00ax-evaluation-methodology.docx
	
	\bibitem{11ay_evaluation} L. Cariou {\it et al}, ``11ay evaluation methodology,'' IEEE 802.11-15/0866r4, May. 2016.
	
	\bibitem{11bf_Ch1} M. Zhang, R. Du, X. Peng, C. Liu, Y. Sun, D. K. Tan, R. Wang, S. Wang, and X. Li, ``Discussion of channel model for WLAN sensing,'' IEEE 802.11-20/0906r0, Jun. 2020. [Online] Available:  https://mentor.ieee.org/802.11/dcn/20/11-20-0906-00-SENS-discussion-of-channel-model-for-wlan-sensing.pptx
	
	\bibitem{11ax_Ch} J. Liu {\it et al}, ``TGax Channel Model Document,'' IEEE 802.11-14/0882r4, Sep. 2014. [Online] Available: https://mentor.ieee.org/802.11/dcn/14/11-14-0882-04-00ax-tgax-channel-model-document.docx
	
	\bibitem{11ay_Ch} A. Maltsev {\it et al}, ``Channel models for ieee 802 11ay,'' IEEE 802.11-15/1150r9, Mar. 2017. [Online] Available: https://mentor.ieee.org/802.11/dcn/15/11-15-1150-09-00ay-channel-models-for-ieee-802-11ay.docx
	
	\bibitem{11bf_Ch2} M.~Zhang, X. Peng, R. Du, C. Liu, Y. Sun, D. K. Tan, R. Wang, S. Wang, and X. Li, ``A brief description of the channel realization generation process,'' IEEE 802.11-20/1334r0, Sep. 2020. [Online] Available: https://mentor.ieee.org/802.11/dcn/20/11-20-1334-00-SENS-a-brief-description-of-the-channel-realization-generation-process.pptx
	
	\bibitem{11bf_Ch3} M.~Zhang {\it et al}, ``Channel models for WLAN sensing systems'', IEEE 802.11-21/0782r3, Aug. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-0782-03-00bf-channel-models-for-wlan-sensing-systems.docx
	
	\bibitem{Ray-Trac} Z. Yun and M. F. Iskander, ``Ray tracing for radio propagation modeling: Principles and applications,'' \textit{IEEE Access}, vol. 3, pp. 1089-1100, Jul. 2015.
	
	\bibitem{11bf_DDHC} Y. Lv, X. Peng, R. Du, M. Hu, H. Xie, R. Wang, S. Wang, Z. Zang, and G. Li, ``Data driving hybrid channel model for WLAN sensing'', IEEE 802.11-21/1241r0, Jul. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-1241-00-00bf-data-driving-hybrid-channel-model-for-wlan-sensing.pptx
	
	\bibitem{DDHC} G. Li, S. Wang, J. Li, R. Wang, F. Liu, M. Zhang, X. Peng, and T. X. Han, ``Rethinking the tradeoff in integrated sensing and communication: Recognition accuracy versus communication rate.'' [Online] Available:https://arxiv.org/abs/2107.09621
	
	\bibitem{11bf_lls} R. Du, M. Zhang, C. Liu, Y. Sun, D. T. K. Pin, E, Au, ``WLAN sensing link level simulation,'' IEEE 802.11-20/1642r0, Oct. 2020. [Online] Available: https://mentor.ieee.org/802.11/dcn/20/11-20-1642-00-00bf-wlan-sensing-link-level-simulation.pptx
	
	\bibitem{11bf_lls_follow_up} R. Du, M. Zhang, X. Peng, D. K. P. Tan, C. Liu, Y. Sun, H. Dai, S. Shi, and W, Wang, ``WLAN sensing link level simulation - follow ups,'' IEEE 802.11-21/0352r1, Mar. 2021. [Online] Available: https://mentor.ieee.org/802.11/dcn/21/11-21-0352-01-00bf-wlan-sensing-link-level-simulation-follow-ups.pptx
	
	\bibitem{11bf_SENS_Proc_Overview} C. d. Silva, C. Beg, C. Chen, O. Au, R. Pushkarna, C. Luo, and O. AboulMagd, ``Proposed Draft Text for SENS Procedure Overview,'' IEEE 802.11-22/0079r2, Feb. 2022. [Online] Available: https://mentor.ieee.org/802.11/dcn/22/11-22-0079-02-00bf-proposed-draft-text-for-sens-procedure-overview.docx
	
	
	
\end{thebibliography}
